ChartInsights: Evaluating Multimodal Large Language Models for Low-Level Chart Question Answering

Chart question answering (ChartQA) tasks play a critical role in interpreting and extracting insights from visualization charts. While recent advancements in multimodal large language models (MLLMs) like GPT-4o have shown promise in high-level ChartQA tasks, such as chart captioning, their effectiveness in low-level ChartQA tasks (e.g., identifying correlations) remains underexplored. In this paper, we address this gap by evaluating MLLMs on low-level ChartQA using a newly curated dataset, ChartInsights, which consists of 22,347 (chart, task, query, answer) covering 10 data analysis tasks across 7 chart types. We systematically evaluate 19 advanced MLLMs, including 12 open-source and 7 closed-source models. The average accuracy rate across these models is 39.8%, with GPT-4o achieving the highest accuracy at 69.17%. To further explore the limitations of MLLMs in low-level ChartQA, we conduct experiments that alter visual elements of charts (e.g., changing color schemes, adding image noise) to assess their impact on the task effectiveness. Furthermore, we propose a new textual prompt strategy, Chain-of-Charts, tailored for low-level ChartQA tasks, which boosts performance by 14.41%, achieving an accuracy of 83.58%. Finally, incorporating a visual prompt strategy that directs attention to relevant visual elements further improves accuracy to 84.32%.

==> secs/apdx.tex <==
\newpage
\section{Appendix}
\subsection{Supplemental Material}
We provide the dataset, code and evaluation logs for review, which are available at: \url{https://anonymous.4open.science/r/ChartInsights-D43E}

% \subsection{Ranking List on \tdataset}
% \subsubsection{Ranking List on Chart Type}
% \subsubsection{Ranking list on Question Type}

% \subsection{MLLMs Details}

==> secs/overview.tex <==
%!TEX root = ../main.tex
\section{\tdataset Construction}
\label{sec:overview}

In this section, we will first discuss the design goals for curating datasets for low-level tasks (Section~\ref{sub:datagoal}).
We will then provide details of constructing \tdataset (Section~\ref{subsec:construct}).
%We will close this section by elaborating on the characteristics of \tdataset  (Section~\ref{sub:dataoverview}).

\subsection{Design Goals for \tdataset}
\label{sub:datagoal}

\begin{figure*}[t!]
	\centering
 	\includegraphics[width=\textwidth]{figs/workflow.pdf}
	\caption{The Pipeline for \tdataset Construction}
	\label{fig:workflow}
\end{figure*}

\paragraph{G1: Supporting Low-level Data Analysis Tasks.} 
Our first goal is to facilitate the support of 10 low-level data analysis tasks~\cite{DBLP:conf/infovis/AmarES05, lowleveltasks}.  This focus addresses a critical gap in existing ChartQA datasets, which often overlook the granularity required to fully understand and interact with the data presented in charts.

%\nan{It seems that evaluating textual prompt variants and text + visual prompts are missing in the design goals.}

\paragraph{G2: Evaluating Visual and Textual Variants on Charts.}
We highlight the critical role of visual variants (\textit{e.g.} color, size, shape) in data visualizations, which are key to conveying and interpreting information effectively. Despite their importance, these variants are often neglected in existing ChartQA datasets and evaluations. Our goal is to address this issue by incorporating a diverse array of visual variants, including varying chart elements, image quality, and visual prompts. In addition, we also want to investigate the impact of different textual prompts on the low-level analysis task.

\paragraph{G3: Making Metadata Available.}
The third goal tackles the prevalent issue of inaccessible data and metadata in current ChartQA datasets. By offering comprehensive access to each chart's metadata, such as the source data, chart type, and visual element specifics (like color schemes and labels), our dataset enhances analytical depth into chart design's impact on ChartQA performance.

%\begin{figure*}[t!]
%\vspace{-1em}
%\centering
%\includegraphics[width=\textwidth]{figs/tasks.pdf}
%\vspace{-1em}
%	\caption{10 Low-level Data Analysis Tasks over 7 Types of Charts}
%	\label{fig:tasks}
%\end{figure*}


%\paragraph{Task Taxonomy on Charts.}
%Tasks in previous benchmarks were mostly redundant and monotonous, making it unlikely to comprehensively evaluate the MLLMs' ability to understand charts. To address this,  we categorize users' understanding of charts into three levels, while also dividing chart understanding tasks into 10 types based on Amar et al.~\cite{DBLP:conf/infovis/AmarES05}. Among the three levels of behavior, Analysis (\add{(T1)--(T4)}) behavior typically requires users to absorb current information and produce new information based on it, placing it at the highest level. We categorize Reasoning, Distribution, Find anomaly and correlation under this level. The next two levels are Search and Query. Search tasks may involve known or unknown search target, as well as comparisons with one element to another. Therefore, we categorize Filter, Determine range, and Order under this level. Query tasks typically involve locating or retrieving known elements, so we categorize Retrieval, Find extreme, and Cluster under this level. 
%
%\stab{\tt (T1) Reasoning}: Users need to calculate the aggregate value of two corresponding elements based on the data in the chart and the requirements in the question.
%
%\stab{\tt (T2) Distribution}: This question mainly pertains to scatterplots, where users need to determine the range of distribution for the scatterplot points. 
%
%\stab{\tt (T3) Find Anomaly}: This question requires users to identify values that appear abnormal based on the different values of elements, either visually or through calculation. For example, which bar seems to have an abnormal length in this graph?
%
%\stab{\tt (T4) Correlation}: This problem typically occurs in scatterplots and line charts, where users need to determine the relationship between the changes in elements and the axes. Some questions can be directly obtained visually, but many cases may require some reasoning process.
%
%\stab{\tt (T5) Filter}: In this task, a random value of an element from the current chart is selected as a reference, and users need to filter the remaining elements based on this reference and the requirements in the question. 
%
%\stab{\tt (T6) Determine Range}: Users need to decide the range of values for the chart based on the values of the elements in the chart.
%
%\stab{\tt (T7) Order}: This task involves sorting the elements in the chart. In \dataset, users are asked to arrange the elements in ascending or descending order of value and output the names of the top three elements for each arrangement.
%
%\stab{\tt (T8) Retrieve Value}: This problem includes both retrieving the values of chart elements and retrieving the structure of the chart. Users may be asked to locate the value of a specific element based on some information or answer structural questions such as the number of elements in the chart.
%
%\stab{\tt (T9) Find extremum}: Users need to identify the maximum and minimum values in the chart and return them.
%
%\stab{\tt (T10) Find Cluster}: Users need to return the number of categories of elements in the chart.

% \paragraph{Chart Taxonomy.}
% In the \dataset project, our focus remains on a thorough examination of the most common types of charts, including bar charts, line charts, pie charts, and scatter plots. This choice is grounded on two core considerations. First, these types of charts frequently appear in daily life, serving as vital tools for conveying information across academic reports, business analyses, or media releases. Hence, enhancing  MLLMs for these charts not only holds significant practical applications but also aids the models in more accurately interpreting and generating text content related to these charts.
% The second consideration stems from our belief that dealing with bar and line charts becomes more challenging when the charts contain multiple categories of elements. Compared to single-category charts, multi-element charts are visually more complex and demand an understanding of the relationships between different elements, including comparisons, contrasts, and trends. To address this complexity, we further subdivided bar and line charts into two subtypes each: complex bar charts and common bar charts, as well as complex line charts and common line charts. This subdivision implies that, within \dataset, we actually study six different types of charts: complex bar, common bar, complex line, common line, pie, and scatter plots.





\subsection{\mbox{The Construction Pipeline for \tdataset}}
\label{subsec:construct}

To fulfill our three design goals, our construction process begins with the collection of charts with metadata from existing datasets. Next, we meticulously assign specific low-level data analysis tasks to appropriate chart types. Lastly, we develop diverse textual prompt strategies, along with visual variants and prompts, tailored to each chart. Note that we save all metadata during the construction process, which can make the users customize their dataset based on \tdataset easily.

As shown in Figure~\ref{fig:workflow}, the construction of our \tdataset consists of five steps: {Candidate Charts Selection}, 
{Low-Level Tasks Generation}, 
{Textual Prompts Design}, 
{Visual Variants Generation}, and 
{Visual Prompts Design}.

\paragraph{Step 1: Candidate Charts Selection.}
In order to more comprehensively evaluate the ability of MLLMs on low-level data analysis tasks, and to conduct more detailed and extended experiments, the datasets (tabular data) and visualization charts we collected need to meet the following three requirements: 
First, these datasets should contain the original metadata of the chart such as the underlying data for rendering, allowing us to create customized reasoning tasks based on the metadata data. Second, the charts in these datasets should contain data labels, because the lack of data labels will greatly limit the types of low-level tasks. 
Third, these datasets should contain both simple and complex charts so that the difficulty of the charts is reasonable. 

After considering the above three aspects and the characteristics of existing datasets, we chose to extract charts and corresponding metadata from the two existing datasets, namely ChartQA~\cite{chartqa} and nvBench~\cite{nvbench}. \textcolor{blue}{Here we have searched lots of datasets. We found that recent datasets related to charts are of good quality and diversity. But most of them are lacking in data labels in charts. ~\cite{plotqa,vistext} In other words, MLLMs can not tell the exact number of each element in the chart. We think these charts are not appropriate for low level analysis tasks, because even humans can not handle those tasks without data labels. We found that there are many high-quality multi-category bar charts and line charts in ChartQA, which are not only clear in image quality with numerical labels but also almost all sourced from Statista. Therefore, the multi-category bar charts and line charts in our dataset are all extracted from Statista. We also found that the images in nvBench are all generated using the Vega-Light visualization syntax, which is in line with the mainstream of academic research. However, there are also many  charts in nvBench that are of low quality, such as some bar charts that have 5 x-axis labels but only two or even one with actual values. We believe that charts with multiple zero values like this are also manifestations of low-quality charts, and we choose to filter them out directly.  } Then, we get a total of 2K high-quality charts as well as their metadata as our initial dataset. The initial dataset contains a total of 7 types of charts, namely stacked bar charts, grouped bar charts, basic bar charts, line charts, grouped line charts, scatterplots, and pie charts. 


\begin{figure*}[t!]
	\centering
	\includegraphics[width=\textwidth]{figs/visualvar.pdf}
	\vspace{-2em}
	\caption{Vary Visual Elements on Charts. (a) We vary chart labels, view size, color, and legend in a total of 15 ways. (b) We alter the image quality by adding noise, applying blur, and adjusting brightness.}
	\label{fig:vary_chart_grammar}
\end{figure*}

\paragraph{Step 2: Low-level Tasks Generation.}
Next, we design a set of low-level tasks for the collected charts. We follow the approach of previous works on designing low-level tasks for charts~\cite{visualizationanalysis, DBLP:conf/infovis/AmarES05, lowleveltasks}, resulting in 10 low-level tasks in this paper, as shown in top of Figure~\ref{fig:teaser}.  
We group the 10 low-level tasks into three categories, namely Analysis, Search, and Query, based on their purpose and required reasoning abilities~\cite{visualizationanalysis}.

Next, we should decide which tasks are applicable to which types of charts. We will follow the recommendations on the task-based effectiveness of humans to assign the tasks to each chart type~\cite{lowleveltasks}.
Finally, we have 22,347 (chart, task, question, answer).


\paragraph{Step 3: Question Type Variation.}
%After the step 2, we have 22,347 initial (question, answer) pairs. 
In order to better explore the impact of different types of questions influence the interaction with MLLMs. We have designed 4 question types, namely Fill-in-the-Blank, Multiple-choice, Yes-or-No, and Error Correction questions. 
1) For Fill-in-the-Blank prompt, we maintain the asking method of the initial question and set the answer format for Fill-in-the-Blank prompt; 
2) For Multiple-choice prompt, we still maintain the asking method of the initial question, but at this time we will provide a list of choices for \mllms, which usually contains one correct answer and two wrong answers, and tells \mllms to choose the answer from the options; 
3) For Yes-or-No prompt, we first change the initial question to a true or false question and tell \mllms whether it needs to be answered correctly or Wrong; and
4) For Error Correction prompt, we put the wrong answer into the original question with a certain probability and change it into a statement.

We expand the above 4 textual prompt variants on the 22,347 (chart, task, query, answer), and thus produce 89,388 (chart, task, question, answer) at the end.

\paragraph{Step 4: Visual Variants Generation.}
Visual variants (\textit{e.g.} color, size, shape) of a chart play a key role in delivering insights, but these variants are often overlooked in existing ChartQA datasets and evaluations, and thus we aim to bridge this gap. To this end, we vary the chart elements and add image noise to vary the chart quality.

\etitle{Step 4.1: Varying the Chart Elements.} As shown in Figure~\ref{fig:vary_chart_grammar}(a), we change the visual elements of these charts from four aspects, namely labels, chart scale, element color, and legend.
To achieve this, we sample 5 charts from each category of charts as seeds, resulting in 35 charts.
For varying labels, we enlarge, reduce, and remove the x-axis, y-axis, and data labels, respectively.
For varying view sizes, we enlarge and reduce the chart, respectively.
For varying element color, we change the elements in the chart to the same color or a higher contrast color;
For varying legend, we first add marks to different types of categories, and then delete the colors.
%
Finally, we generate 356 visual variants for 35 charts. These 356 visual variants (charts) are associated with 17,972 textual prompts and cover 10 low-level tasks.

\etitle{Step 4.2: Varying the Image Quality.} 
We add image noise, apply image blur, and adjust the brightness to vary the chart image quality, as shown in Figure~\ref{fig:vary_chart_grammar}(b).
To achieve this, we sample 5 charts from each category of charts as seeds, resulting in 35 charts.
For adding image noise, we choose Gaussian noise and salt and pepper noise;
For applying image blue, we use median blur and Gaussian blur;
For adjusting image brightness, we choose to make the brightness of the chart higher and lower.
Finally, we generate 245 visual variants for 35 charts. These 245 visual variants (charts) are associated with 8,456 textual prompts and cover 10 low-level tasks.





\paragraph{Step 5: Visual Prompts Design.}
Kong et al.~\cite{overlays} presented five types of graphical overlays to enhance users' capabilities in performing data analysis tasks such as extraction and comparison of numerical values. Intuitively, we want to verify whether overlays would have a positive impact on \mllms's performance.
Therefore, we design three types of visual prompts (\textit{i.e.} graphical overlays) for the charts.

We consider three types of visual prompts, as shown in Figure~\ref{fig:visualprompts}.
The first is to directly circle the content in the chart that is highly relevant to the question in handwriting, such as circling the values of the two elements mentioned in the reasoning question.
The second method is regular shapes, which uses regular shapes (such as circles or rectangles) to label elements in the diagram. This makes it easier to use the size of a shape to imply the sequential relationship of elements. For example, use three circles of different sizes to correspond to the three values in the ordering task.
The third way is special design. We design effective visual prompts tailored for different low-level tasks. For example, we use arrows to represent the monotonicity of the trend, for the correlation task. 
To generate the visual prompts, we first sample 35 charts from seven chart types, then apply various visual prompt strategies to them, resulting in 255 charts with different visual prompts. These 255 charts are associated with 1020 questions for 10 low-level tasks.




\section{Ten Low-Level ChartQA Tasks}
\label{app:dataset}

\begin{figure}[t!]
	\centering
	\includegraphics[width=\columnwidth]{figs/chart_dist.pdf}
	\vspace{-.5em}
	\caption{Low-level Tasks Distribution}
	\label{fig:dataset_stat1}
	\vspace{-10px}
\end{figure}

Our \tdataset include 10 low-level data analysis tasks on charts, as shown in Figure~\ref{fig:dataset_stat1}.


\paragraph{T1: Data Retrieval.} This question includes both the retrieval of the value of chart elements and the retrieval of the structure of the chart. Figure~\ref{fig:data_retrieval_example} shows an example. Users will be asked to locate the value of an element based on some information, or they may be asked to answer structural questions such as how many elements there are in the chart.

\begin{figure*}[t!]
	\centering
	\includegraphics[width=\textwidth]{figs/examples/Data_Retrieval_Example.pdf}
	\vspace{-2em}
	\caption{An Example of Data Retrieval Tasks}
\label{fig:data_retrieval_example}
\end{figure*}

\paragraph{T2: Reasoning.} Users need to calculate the aggregate value of multiple elements based on the data in the chart and the requirements of the question.  Figure~\ref{fig:Reasoning_example} shows an example.
\begin{figure*}[t!]
	\centering
	\includegraphics[width=\textwidth]{figs/examples/Reasoning_Example.pdf}
	\vspace{-2em}
	\caption{An Example of Reasoning Tasks}
	\label{fig:Reasoning_example}
\end{figure*}

\paragraph{T3: Filter.} This question will randomly select a value of an element in the current chart as a benchmark, and users need to filter the remaining elements according to this benchmark and the requirements of the question. Figure~\ref{fig:Filter_example} shows an example.

\begin{figure*}[t!]
	\centering
	\includegraphics[width=\textwidth]{figs/examples/Filter_Example.pdf}
	\vspace{-2em}
	\caption{An Example of Filter Tasks}
	\label{fig:Filter_example}
\end{figure*}
\paragraph{T4: Determine Range.} This question requires users to determine the value range of the chart based on the values of the elements in the chart. Figure~\ref{fig:Determine_Range_example} shows an example.
\begin{figure*}[t!]
	\centering
	\includegraphics[width=\textwidth]{figs/examples/Determine_Range_Example.pdf}
	\vspace{-2em}
	\caption{An Example of Determine Range Tasks}
	\label{fig:Determine_Range_example}
\end{figure*}

\paragraph{T5: Cluster.} This question requires users to return the number of categories of elements in the chart. Figure~\ref{fig:Cluster_example} shows an example.
\begin{figure*}[t!]
	\centering
	\includegraphics[width=\textwidth]{figs/examples/Cluster_Example.pdf}
	\vspace{-2em}
	\caption{An Example of Cluster Tasks}
	\label{fig:Cluster_example}
\end{figure*}

\paragraph{T6: Find Extreme.} This question requires users to find the maximum and minimum values in the chart and return them. Figure~\ref{fig:Find_extreme_example} shows an example.
\begin{figure*}[t!]
	\centering
	\includegraphics[width=\textwidth]{figs/examples/Find_Extreme_Example.pdf}
	\vspace{-2em}
	\caption{An Example of Find Extreme Tasks}
	\label{fig:Find_extreme_example}
\end{figure*}

\paragraph{T7: Correlation.} This question usually appears in scatter and line charts, where users need to determine the relationship between the changes in the elements in the chart and the axes. Some questions can be answered visually, but many require a reasoning process. Figure~\ref{fig:Correlation_example} shows an example.
\begin{figure*}[t!]
	\centering
	\includegraphics[width=\textwidth]{figs/examples/Correlation_Example.pdf}
	\vspace{-2em}
	\caption{An Example of Correlation Tasks}
	\label{fig:Correlation_example}
\end{figure*}

\paragraph{T8: Find Anomaly.} This question requires users to identify values that appear to be anomalies based on their different values, either visually or through calculation. Figure~\ref{fig: Find_Anomaly_example} shows an example.
\begin{figure*}[t!]
	\centering
	\includegraphics[width=\textwidth]{figs/examples/Find_Anomaly_Example.pdf}
	\vspace{-2em}
	\caption{An Example of Find Anomaly Tasks}
	\label{fig: Find_Anomaly_example}
\end{figure*}

\paragraph{T9: Order.} This question involves sorting the elements in the chart. In ChartInsights, users will be asked to sort the elements in ascending or descending order of value and output the names of the top three elements for each type of sorting. Figure~\ref{fig: Order_example} shows an example.
\begin{figure*}[t!]
	\centering
	\includegraphics[width=\textwidth]{figs/examples/Order_Example.pdf}
	\vspace{-2em}
	\caption{An Example of Order Tasks}
	\label{fig: Order_example}
\end{figure*}

\paragraph{T10: Distribution.} This question is mainly for scatter plots, where users need to determine the distribution range of the dots. Figure~\ref{fig: Distribution_example} shows an example.

\begin{figure*}[t!]
	\centering
	\includegraphics[width=\textwidth]{figs/examples/Distribution_Example.pdf}
	\vspace{-2em}
	\caption{An Example of Distribution Tasks}
	\label{fig: Distribution_example}
\end{figure*}

%\paragraph{Training Set and Testing Set.}
%We randomly split the \dataset into a training set (80\%) and a testing set (20\%). We ensure that both training and test sets include 7 chart types and 10 low-level tasks and follow similar distributions. The training set can be utilized to fine-tune the \mllms. 
%The training set contains 71,863 (charts, tasks, questions, answers) samples associated with 1600 charts.
%The testing set consists of 17,552 (charts, tasks, questions, answers) samples associated with 400 charts.
%We use the testing set to evaluate the effectiveness of GPT-4V on low-level analysis tasks.
%\add{Note that we do not fine-tune any MLLMs; instead, we evaluate the ``off-the-shelf'' GPT-4V using only the testing set..}


